Search for the rare decay $D^+ \to D^0 e^+\nu_e$

We search for the rare decay $D^+\to D^0 e^+\nu_{e}$, using a data set with an integrated luminosity of 2.93 $\rm fb^{-1}$ collected at $\sqrt{s}=3.773$ GeV with the BESIII detector operating at the BEPCII storage rings. No signals are observed. We set the upper limit on the branching fraction for $D^+\to D^0 e^+\nu_e$ to be $1.0\times 10^{-4}$ at the 90\% confidence level.

==> signal.tex <==
\section{Signal Extraction}
\label{sec:signal}
\vspace{-0.4cm}
To extract the resonance parameters and yield of $Z_c(3885)^-$ in the $(D\bar{D}^*)^-$ mass spectrum,
both processes are fitted simultaneously with an unbinned maximum likelihood method
using two different data samples at $\sqrt{s}$=4.23~GeV and $\sqrt{s}$=4.26~GeV.
The $(D\bar{D}^*)^-$ invariant mass distribution is described as
the sum of two probability density functions (PDFs) representing the signal and background.
The signal PDF is given by
\begin{eqnarray}
\begin{aligned}
\mbox{PDF}(m_{D\bar{D}^*}) = \frac{[S(m_{D\bar{D}^*})\otimes R]\epsilon(m_{D\bar{D}^*})}
{\int[S(m_{D\bar{D}^*})\otimes R]\epsilon(m_{D\bar{D}^*})dm_{D\bar{D}^*}},
\end{aligned}
\end{eqnarray}
where the integral is performed over the fit range of the $(D\bar{D}^*)^-$ mass spectrum,
$S(m_{D\bar{D}^*})\otimes R$ is the signal term convolved with the mass resolution,
and $\epsilon(m_{D\bar{D}^*})$ is the reconstruction efficiency.
The background PDF is parameterized by phase space MC simulation.
The signal and background yields and the mass and width of $Z_c(3885)^-$ are determined in the fit.
The mass and width of $Z_c(3885)^-$ are constrained to be the same for both processes.
\subsection{Signal Term}
\vspace{-0.4cm}
The process $e^+e^-\to\pi^{+}Z_c(3885)^{-}$ with $Z_c(3885)^{-}\to \rm{I}$
is described with phase space generalized
for the angular momentum $L$ of the $\pi^{+}-Z_c(3885)^{-}$ system,
where I denotes $D^-D^{*0}$ (labeled as $a$) and $D^0D^{*-}$ (labeled as $b$).
The $Z_c(3885)^{-}$ is described by a mass dependent width Breit-Wigner (MDBW)
parameterization~\cite{PRL96-102002}.
\begin{eqnarray}
\begin{aligned}
&S_{\rm{I}}(m_{D\bar{D}^*})\propto dN/dm_{D\bar{D}^*}\\
&\quad\propto (\kappa^*)^{2L+1}f^2_{L}(\kappa^*)|BW_{\rm{I}}(m_{D\bar{D}^*})|^2,
\end{aligned}
\label{sigpdf}
\end{eqnarray}
where $\kappa^*$ is the momentum of $Z_c(3885)^-$ in the $e^+e^-$ rest frame,
$f_{L}(\kappa^*)$ is the Blatt-Weisskopf barrier factor~\cite{fRi},
\begin{eqnarray}
&BW_{\rm{I}}(m_{D\bar{D}^*})\propto
&\frac{\sqrt{m_{D\bar{D}^*}\Gamma_{\rm{I}}}}
{m^2_{Z_c}-m^2_{D\bar{D}^*}-i\frac{1}{2}m_{Z_c}(\Gamma_{a}+\Gamma_{b})},
\label{RBW}
\end{eqnarray}
$\Gamma_{\rm{I}} = \Gamma_{Z_c}[q_{\rm{I}}^*/q_{\rm{I}}^0]^{2\ell+1}[m_{Z_c}/m_{D\bar{D}^*}][f_{\ell}(q_{\rm{I}}^*)/f_{\ell}(q_{\rm{I}}^0)]^2$,
$q_{\rm{I}}^*$ is the $D$ momentum in the $Z_c(3885)^-$ rest frame,
$\ell$ is the angular momentum of the $(DD^{*})^-$ system, and $q_{\rm{I}}^0 \equiv q_{\rm{I}}^*(m_{Z_c})$.
In the fit, $m_{Z_c}$ and $\Gamma_{Z_c}$ are free parameters,
while $L =0$ and $\ell = 0$ are fixed according to the analysis of angular distributions below.
Parameters of the resolution and efficiency functions, obtained from MC and described below, are fixed in the fit.

\subsection{Reconstruction Efficiency and Mass Resolution}
\vspace{-0.4cm}
In order to obtain the reconstruction efficiency and mass resolution,
we generate a set of MC samples for $e^+e^-\to\pi^+Z^-_c~(Z^-_c\to(D\bar{D}^*)^-)$,
each with a fixed mass value, zero width and $J^P=1^+$ of the $Z^-_c$,
and subject these MC samples to the same event selection criteria.
The isospin channel $e^+e^-\to\pi^+D^0D^{*-}$ ($D^{*-} \to D^-\pi^0$) can feed into the $\pi^+D^-D^0$-tagged process.
We therefore generate two corresponding MC samples by assuming the same decay branching fraction between the process
$Z_c^-\to D^-D^{*0}$ and $Z_c^-\to D^0D^{*-}$.
The reconstruction efficiency is estimated using the sum of the two MC samples, as shown in Fig.~\ref{eff_curve}.

\begin{figure*}[htbp]
\centering
\begin{minipage}[b]{0.45\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=Eff_4230_D0D0.eps}
\put(-50,120){\bf\boldmath (a)}
\end{minipage}
\begin{minipage}[b]{0.45\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=Eff_4230_D0Dm.eps}
\put(-50,120){\bf\boldmath (b)}
\end{minipage}
\begin{minipage}[b]{0.45\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=Eff_4260_D0D0.eps}
\put(-50,120){\bf\boldmath (c)}
\end{minipage}
\begin{minipage}[b]{0.45\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=Eff_4260_D0Dm.eps}
\put(-50,120){\bf\boldmath (d)}
\end{minipage}
\caption{Distributions of the efficiency versus $M(D\bar{D}^*)$
for ((a) and (c)) $\pi^+D^0\bar{D}^0$-tagged and ((b) and (d)) $\pi^+D^-D^0$-tagged processes
at ((a) and (b)) $\sqrt{s}$=4.23~GeV and ((c) and (d)) $\sqrt{s}$=4.26~GeV.
The dots with error bars are the efficiencies determined from MC.
The curves show the fits with a piecewise linear function.}
\label{eff_curve}
\end{figure*}

MC samples for $e^+e^-\to\pi^+Z^-_c~(Z^-_c\to(D\bar{D}^*)^-)$ are used to determine the mass resolution.
The mass and width of $Z_c$ are set to be 3890~MeV/$c^2$ and 0~MeV, respectively.
The mass resolution for the $\pi^+D^0\bar{D}^0$-tagged process is described
by a Crystal Ball (CB) function~\cite{CB}.
Since the $\pi^+D^-D^0$-tagged process contains two isospin processes,
the mass resolution is represented by a sum of two CB functions with a common mean and different widths.
The fit results for both processes are shown in Fig.~\ref{resolution}.
The resolution for the $\pi^+D^0\bar{D}^0$-tagged process is determined by
the fit to be 1.1$\pm$0.1~MeV/$c^2$,
while the resolution for the $\pi^+D^-D^0$-tagged process is
calculated to be 2.2$\pm$0.1~MeV/$c^2$ using the equation $f_1 \sigma_1 + (1-f_1)\sigma_2$,
where $\sigma_1$ and $\sigma_2$ are the individual widths of each of the two CB functions and
$f_1$ is the fractional area of the first CB function.

\begin{figure*}[hbtp]
\centering
\begin{minipage}[b]{0.45\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=Res_4230_D0D0.eps}
\put(-50,120){\bf\boldmath (a)}
\end{minipage}
\begin{minipage}[b]{0.45\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=Res_4230_D0Dm.eps}
\put(-50,120){\bf\boldmath (b)}
\end{minipage}
\begin{minipage}[b]{0.45\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=Res_4260_D0D0.eps}
\put(-50,120){\bf\boldmath (c)}
\end{minipage}
\begin{minipage}[b]{0.45\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=Res_4260_D0Dm.eps}
\put(-50,120){\bf\boldmath (d)}
\end{minipage}
\caption{Fits to the mass resolution at 3890~MeV for
((a) and (c)) $\pi^+D^0\bar{D}^0$-tagged and ((b) and (d)) $\pi^+D^-D^0$-tagged processes
at ((a) and (b)) $\sqrt{s}$=4.23~GeV and ((c) and (d)) $\sqrt{s}$=4.26~GeV.
The dots with error bars show the distributions of mass resolutions obtained from MC,
the curves show the fits.}
\label{resolution}
\end{figure*}

\subsection{Fit Results }
\vspace{-0.4cm}
As shown in Fig.~\ref{sig_fit}, we perform a simultaneous fit to the $M(D\bar{D}^*)$ distributions
for the $\pi^+D^0\bar{D}^0$-tagged and $\pi^+D^-D^0$-tagged processes
with $\sqrt{s}$=4.23~GeV and $\sqrt{s}$=4.26~GeV data samples.
The statistical significance of $Z_c(3885)^-$, estimated by the difference of log-likelihood
values with and without signal terms in the fit, is greater than 10$\sigma$.
The mass and width of $Z_c(3885)^-$ are fitted to be
$M_{Z_c(3885)}$ = (3890.3$\pm$0.8)~MeV/$c^2$ and $\Gamma_{Z_c(3885)}$ = (31.5$\pm$3.3)~MeV,
where the errors are statistical only.
Since the resulting mass and width might be different from the actual resonance properties
due to the parameterization function of $Z_c(3885)$,
we calculate the pole position ($P = M_{\rm{pole}} -i\Gamma_{\rm{pole}}/2$) of $Z_c(3885)$
which is the complex number where the denominator of $BW_{\rm{I}}(m_{D\bar{D}^*})$ is zero,
and regard $M_{\rm{pole}}$ and $\Gamma_{\rm{pole}}$ as the final result.
The corresponding pole mass ($M_{\rm{pole}}$) and width ($\Gamma_{\rm{pole}}$) of
$Z_c(3885)$ are $M_{\rm{pole}}$ = (3881.7$\pm$1.6)~MeV/$c^2$ and $\Gamma_{\rm{pole}}$ = (26.6$\pm$2.0)~MeV, respectively.

\subsection{Angular Distribution}
\vspace{-0.4cm}
The quantum number $J^P$ assignment for $Z_c(3885)^-$ is investigated by examining the distribution of \textbar \rm{cos}$\theta_{\pi}$\textbar,
where $\theta_\pi$ is the $\pi^+$ polar angle relative to the beam direction in the center-of-mass frame.
If $J^P=1^+$, the relative orbital angular momentum of the $\pi^+$-$Z_c(3885)^{-}$ system could be either $S$-wave or $D$-wave.
If we neglect the small contribution of $D$-wave due to the closeness of the threshold,
the \textbar \rm{cos}$\theta_{\pi}$\textbar ~distribution is expected to be flat.
If $J^P=0^-$ ($1^-$), the $\pi^{+}$-$Z_c(3885)^{-}$ system occurs via a $P$-wave
and the \textbar \rm{cos}$\theta_{\pi}$\textbar ~is expected to follow $\rm{sin}^2\theta_{\pi}$ (1+$\rm{cos}^2\theta_{\pi}$) distribution.

The \textbar \rm{cos}$\theta_{\pi}$\textbar ~distribution of data is plotted with
the efficiency corrected signal yield of combined data samples at $\sqrt{s}$=4.23~GeV and $\sqrt{s}$=4.26~GeV
in ten \textbar \rm{cos}$\theta_{\pi}$\textbar ~bins,
where the signal yields in different bin are extracted with the same simultaneous fit method described above.
Figures~\ref{Eff_cospi} (a) and (b) show the \textbar \rm{cos}$\theta_{\pi}$\textbar ~distribution for
$\pi^+D^0\bar{D}^0$-tagged process and $\pi^+D^-D^0$-tagged process, respectively.
The data agrees well with the flat distribution expected
for $J^P=1^+$ ($\chi^2$/NDF = 16.5/9 for the $\pi^+D^0\bar{D}^0$-tagged process
and 12.8/9 for the $\pi^+D^-D^0$-tagged process) and disagrees with the $\rm{sin}^2\theta_{\pi}$
distribution expected for $J^P=0^-$ ($\chi^2$/NDF = 103.1/9 for the $\pi^+D^0\bar{D}^0$-tagged process
and 104.9/9 for the $\pi^+D^-D^0$-tagged process) and $J^P=1^-$
($\chi^2$/NDF = 106.3/9 for the $\pi^+D^0\bar{D}^0$-tagged process
and 104.9/9 for the $\pi^+D^-D^0$-tagged process), where NDF is the number of degrees of freedom in the fit.

\begin{figure*}[htbp]
\centering
\begin{minipage}[b]{0.48\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=plot_angular_D0D0.eps}
\put(-50,120){\bf\boldmath (a)}
\end{minipage}
\begin{minipage}[b]{0.48\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=plot_angular_D0Dm.eps}
\put(-50,120){\bf\boldmath (b)}
\end{minipage}
\caption{Fits to \textbar \rm{cos}$\theta_{\pi}$\textbar\ distributions for (a) $\pi^+D^0\bar{D}^0$-tagged
and (b) $\pi^+D^-D^0$-tagged processes.
The dots with error bars show the combined data corrected for detection efficiency at $\sqrt{s}$=4.23~GeV and $\sqrt{s}$=4.26~GeV,
the solid lines show the fits using $J^P=1^+$ hypothesis,
and the dashed and dotted curves are for the fits with $J^P=0^-$ and $J^P=1^-$ hypothesis, respectively.}
\label{Eff_cospi}
\end{figure*}

\subsection{Born Cross Section}
\vspace{-0.4cm}
For the $\pi^+D^0\bar{D}^0$-tagged process, the Born cross section
times the $(D\bar{D}^*)^-$ branching fraction of $Z_c(3885)^-$ ($\sigma\times Br$) can be calculated by
%\begin{widetext}
\begin{eqnarray}
\begin{aligned}
\sigma(e^+e^-\to\pi^{\pm}Z_c(3885)^{\mp})\times Br(Z_c(3885)^{\mp}\to (D\bar{D}^*)^{\mp})\\
= \frac{N}{\mathcal{L}(1+\delta^{r})(1+\delta^{v})
\sum_{\substack {i,j}}\epsilon_{ij}Br_{i}Br_{j}Br(D^{*-}\to\pi^-\bar{D}^0)I},
\label{eq1}
\end{aligned}
\end{eqnarray}
%\end{widetext}
where $N$ is the signal yield, $\mathcal{L}$ is the integrated luminosity,
$\epsilon_{ij}$ is the signal efficiency for the $\pi^+D^0\bar{D}^0$-tagged process listed in Table~\ref{tab:eff_D0D0}
of Appendix~\ref{sec:appA},
where the subscripts $i, j = 0 \ldots 3$ denote the neutral $D$ final state,
$Br_{i}$ is the individual branching fraction for $D$ decay from PDG~\cite{pdg},
the radiative correction factor ($1+\delta^{r}$) is determined by
the measurement of the line shape of $\sigma(e^+e^-\to\pi D\bar{D}^*)$~\cite{PRL112-022001},
the vacuum polarization factor ($1+\delta^{v}$) is considered in the MC simulation~\cite{EPJC-66-585}
and $I = Br(Z_c(3885)^-\to D^0D^{*-})/Br(Z_c(3885)^-\to (D\bar{D}^*)^-)$ = 0.5, assuming isospin symmetry.
The value of all above variables are listed in Table~\ref{tab:cros}.

Since the $\pi^+D^-D^0$-tagged process contains two processes of
$Z_c(3885)^-\to D^-D^{*0}$ with $D^{*0}\to\pi^0D^0$ (labeled as $\alpha$)
and $Z_c(3885)^-\to D^0D^{*-}$ with $D^{*-}\to\pi^0D^-$ (labeled as $\beta$),
the Born cross section times the $(D\bar{D}^*)^-$ branching fraction of $Z_c(3885)^-$ can be given by
\begin{widetext}
\begin{eqnarray}
\begin{aligned}
&\sigma(e^+e^-\to\pi^{\pm}Z_c(3885)^{\mp})\times Br(Z_c(3885)^{\mp}\to (D\bar{D}^*)^{\mp})\\
&= \frac{N}{\mathcal{L}(1+\delta^{r})(1+\delta^{v})
(\sum_{\substack {i,j}}\epsilon^{\alpha}_{ij}Br_{i}Br_{j}Br(D^{*0}\to\pi^0D^0)
+\sum_{\substack {i,j}}\epsilon^{\beta}_{ij}Br_{i}Br_{j}Br(D^{*-}\to\pi^0D^-))I},\\
\end{aligned}
\end{eqnarray}
\end{widetext}
where $\epsilon^{\alpha}_{ij}$ and $\epsilon^{\beta}_{ij}$ are the signal efficiency for the two $\pi^+D^-D^0$-tagged processes,
listed in Table~\ref{tab:eff_D0Dma} and~\ref{tab:eff_D0Dmb} of Appendix~\ref{sec:appA},
the subscripts $i$ and $j$ denote the $D^-$ and $D^0$ final states,
respectively, with $i = A \ldots F$ and $j = 0 \ldots 3$,
$Br(D^{*0}\to\pi^0D^0)$ = (61.9$\pm$2.9)\% and $Br(D^{*-}\to\pi^0D^-)$ = (30.7$\pm$0.5)\%~\cite{pdg}.
The value of all above variables are listed in Table~\ref{tab:cros}.

We also add a $Z_c(4020)^-$ in the fit with mass and width fixed to the BESIII measurement~\cite{PRL111-242001}.
The fit prefers the presence of a $Z_c(4020)^-$ with a statistical significance of 1.0$\sigma$.
We determine the upper limit on $\sigma\times Br$ at the 90\% confidence level (C.L.),
where the probability density function from the fit is smeared by a Gaussian function
with a standard deviation of the relative systematic error in the $\sigma\times Br$ measurement.
We obtain $\sigma(e^+e^-\to\pi^{\pm}Z_c(4020)^{\mp})\times Br(Z_c(4020)^{\mp}\to (DD^*)^{\mp})<$
18~pb at $\sqrt{s}$=4.23~GeV and $<$15~pb at $\sqrt{s}$=4.26~GeV, respectively, at 90\% C.L..

\begin{table*}[htbp]
\begin{center}
\caption{Summary of the product of Born cross sections times the $(D\bar{D}^*)^-$ branching
fraction of $Z_c(3885)^-$ ($\sigma\times Br$), the errors are statistical only.
}
\begin{tabular}{lcccc}
\hline
\hline
\multirow{2}{*}{}
& \multicolumn{2}{c}{$\pi^+D^0\bar{D}^0$-tagged process}
& \multicolumn{2}{c}{$\pi^+D^-D^0$-tagged process}
\\
\cline{2-3}
\cline{4-5}
& 4.23~GeV
& 4.26~GeV
& 4.23~GeV
& 4.26~GeV
\\
\hline
\hline
$N$			      &  384$\pm$30  &   207$\pm$18  &  418$\pm$34  & 239$\pm$22  \\
$\mathcal{L}$ (pb$^{-1}$)     &  1091.7        &   825.7         &  1091.7        & 825.7         \\
1+$\delta^{r}$		      &  0.89 & 0.92     & 0.89 & 0.92       \\
1+$\delta^{v}$		      &  1.056 & 1.054                   &     1.056 & 1.054                   \\
$\sigma\times Br$ (pb)	      &  147.5$\pm$11.5 & 109.2$\pm$9.7 & 136.6$\pm$11.0 & 107.5$\pm$9.7  \\
\hline
\hline
\end{tabular}
\label{tab:cros}
\end{center}
\end{table*}

